An LLM-based Readability Measurement for Unit Tests' Context-aware Inputs

Automated test techniques usually generate unit tests with higher code coverage than manual tests. However, the readability of automated tests is crucial for code comprehension and maintenance. The readability of unit tests involves many aspects. In this paper, we focus on test inputs. The central limitation of existing studies on input readability is that they focus on test codes alone without taking the tested source codes into consideration, making them either ignore different source codes' different readability requirements or require manual efforts to write readable inputs. However, we observe that the source codes specify the contexts that test inputs must satisfy. Based on such observation, we introduce the \underline{C}ontext \underline{C}onsistency \underline{C}riterion (a.k.a, C3), which is a readability measurement tool that leverages Large Language Models to extract primitive-type (including string-type) parameters' readability contexts from the source codes and checks whether test inputs are consistent with those contexts. We have also proposed EvoSuiteC3. It leverages C3's extracted contexts to help EvoSuite generate readable test inputs. We have evaluated C3's performance on $409$ \java{} classes and compared manual and automated tests' readability under C3 measurement. The results are two-fold. First, The Precision, Recall, and F1-Score of C3's mined readability contexts are \precision{}, \recall{}, and \fone{}, respectively. Second, under C3's measurement, the string-type input readability scores of EvoSuiteC3, ChatUniTest (an LLM-based test generation tool), manual tests, and two traditional tools (EvoSuite and Randoop) are $90\%$, $83\%$, $68\%$, $8\%$, and $8\%$, showing the traditional tools' inability in generating readable string-type inputs.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tab/bugs.tex <==
\begin{table*}[tbp]
    \centering
    \tiny

    \caption{\mynewcontent{6}{Bug detection summary for each strategy with WS}}\label{tab:ws_bugs}
       \begin{tabular}{llccc|ccc|ccc|ccc|ccc}
\toprule
Project & Bugs & \nrcols{3}{Smart Selection} & \nrcols{3}{Original Combination}  & \nrcols{3}{Branch Coverage} & \nrcols{3}{BC-EC-MC} & \nrcols{3}{SSWS} \\
\cmidrule(l{1pt}r{1pt}){3-5}
\cmidrule(l{1pt}r{1pt}){6-8}
\cmidrule(l{1pt}r{1pt}){9-11}
\cmidrule(l{1pt}r{1pt}){12-14}
\cmidrule(l{1pt}r{1pt}){15-17}
 & & Detected & Detect$\%$ & Fail$\%$ & Detected & Detect$\%$ & Fail$\%$ & Detected & Detect$\%$ & Fail$\%$ & Detected & Detect$\%$ & Fail$\%$ & Detected & Detect$\%$ & Fail$\%$  \\
\midrule


 Chart  & \significant{\num{24}} & \significant{\num{19}} & \significant{\num{0.57}} & \significant{\num{0.05}}  & \significant{\num{17}} & \significant{\num{0.57}} & \significant{\num{0.07}} & \significant{\num{18}} & \significant{\num{0.56}} & \significant{\num{0.05}} & \significant{\num{15}} & \significant{\num{0.48}} & \significant{\num{0.06}} & \significant{\num{16}} & \significant{\num{0.55}} & \significant{\num{0.10}}  \\



\tabprojectlinespace 


 Cli  & \significant{\num{28}} & \significant{\num{14}} & \significant{\num{0.42}} & \significant{\num{0.01}}  & \significant{\num{14}} & \significant{\num{0.41}} & \significant{\num{0.03}} & \significant{\num{15}} & \significant{\num{0.41}} & \significant{\num{0.01}} & \significant{\num{12}} & \significant{\num{0.38}} & \significant{\num{0.00}} & \significant{\num{15}} & \significant{\num{0.38}} & \significant{\num{0.00}}  \\



\tabprojectlinespace 


 Closure  & \significant{\num{38}} & \significant{\num{8}} & \significant{\num{0.16}} & \significant{\num{0.17}}  & \significant{\num{9}} & \significant{\num{0.14}} & \significant{\num{0.14}} & \significant{\num{5}} & \significant{\num{0.07}} & \significant{\num{0.06}} & \significant{\num{10}} & \significant{\num{0.15}} & \significant{\num{0.21}} & \significant{\num{7}} & \significant{\num{0.12}} & \significant{\num{0.16}}  \\



\tabprojectlinespace 


 Compress  & \significant{\num{29}} & \significant{\num{13}} & \significant{\num{0.27}} & \significant{\num{0.08}}  & \significant{\num{13}} & \significant{\num{0.26}} & \significant{\num{0.05}} & \significant{\num{15}} & \significant{\num{0.29}} & \significant{\num{0.03}} & \significant{\num{11}} & \significant{\num{0.23}} & \significant{\num{0.06}} & \significant{\num{9}} & \significant{\num{0.25}} & \significant{\num{0.05}}  \\



\tabprojectlinespace 


 Csv  & \significant{\num{8}} & \significant{\num{7}} & \significant{\num{0.67}} & \significant{\num{0.03}}  & \significant{\num{6}} & \significant{\num{0.71}} & \significant{\num{0.09}} & \significant{\num{6}} & \significant{\num{0.57}} & \significant{\num{0.00}} & \significant{\num{6}} & \significant{\num{0.64}} & \significant{\num{0.00}} & \significant{\num{6}} & \significant{\num{0.69}} & \significant{\num{0.09}}  \\



\tabprojectlinespace 


 Gson  & \significant{\num{14}} & \significant{\num{5}} & \significant{\num{0.36}} & \significant{\num{0.01}}  & \significant{\num{5}} & \significant{\num{0.36}} & \significant{\num{0.01}} & \significant{\num{5}} & \significant{\num{0.31}} & \significant{\num{0.01}} & \significant{\num{5}} & \significant{\num{0.36}} & \significant{\num{0.03}} & \significant{\num{5}} & \significant{\num{0.32}} & \significant{\num{0.04}}  \\



\tabprojectlinespace 


 JacksonCore  & \significant{\num{22}} & \significant{\num{13}} & \significant{\num{0.41}} & \significant{\num{0.04}}  & \significant{\num{11}} & \significant{\num{0.37}} & \significant{\num{0.04}} & \significant{\num{14}} & \significant{\num{0.51}} & \significant{\num{0.05}} & \significant{\num{11}} & \significant{\num{0.46}} & \significant{\num{0.08}} & \significant{\num{13}} & \significant{\num{0.46}} & \significant{\num{0.01}}  \\



\tabprojectlinespace 


 JacksonDatabind  & \significant{\num{75}} & \significant{\num{30}} & \significant{\num{0.27}} & \significant{\num{0.11}}  & \significant{\num{27}} & \significant{\num{0.23}} & \significant{\num{0.12}} & \significant{\num{22}} & \significant{\num{0.20}} & \significant{\num{0.11}} & \significant{\num{26}} & \significant{\num{0.26}} & \significant{\num{0.14}} & \significant{\num{31}} & \significant{\num{0.27}} & \significant{\num{0.13}}  \\



\tabprojectlinespace 


 JacksonXml  & \significant{\num{6}} & \significant{\num{2}} & \significant{\num{0.23}} & \significant{\num{0.10}}  & \significant{\num{2}} & \significant{\num{0.23}} & \significant{\num{0.02}} & \significant{\num{2}} & \significant{\num{0.33}} & \significant{\num{0.03}} & \significant{\num{2}} & \significant{\num{0.32}} & \significant{\num{0.07}} & \significant{\num{2}} & \significant{\num{0.28}} & \significant{\num{0.07}}  \\



\tabprojectlinespace 


 Jsoup  & \significant{\num{58}} & \significant{\num{21}} & \significant{\num{0.28}} & \significant{\num{0.06}}  & \significant{\num{20}} & \significant{\num{0.31}} & \significant{\num{0.04}} & \significant{\num{20}} & \significant{\num{0.27}} & \significant{\num{0.01}} & \significant{\num{22}} & \significant{\num{0.29}} & \significant{\num{0.06}} & \significant{\num{22}} & \significant{\num{0.29}} & \significant{\num{0.06}}  \\



\tabprojectlinespace 


 JxPath  & \significant{\num{12}} & \significant{\num{6}} & \significant{\num{0.38}} & \significant{\num{0.28}}  & \significant{\num{6}} & \significant{\num{0.30}} & \significant{\num{0.13}} & \significant{\num{7}} & \significant{\num{0.40}} & \significant{\num{0.09}} & \significant{\num{7}} & \significant{\num{0.33}} & \significant{\num{0.22}} & \significant{\num{5}} & \significant{\num{0.22}} & \significant{\num{0.17}}  \\



\tabprojectlinespace 


 Lang  & \significant{\num{44}} & \significant{\num{23}} & \significant{\num{0.40}} & \significant{\num{0.04}}  & \significant{\num{19}} & \significant{\num{0.35}} & \significant{\num{0.02}} & \significant{\num{22}} & \significant{\num{0.44}} & \significant{\num{0.01}} & \significant{\num{24}} & \significant{\num{0.50}} & \significant{\num{0.01}} & \significant{\num{29}} & \significant{\num{0.48}} & \significant{\num{0.03}}  \\



\tabprojectlinespace 


 Math  & \significant{\num{2}} & \significant{\num{1}} & \significant{\num{0.45}} & \significant{\num{0.00}}  & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}} & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}} & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}} & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}}  \\



\midrule


 Overall  & \significant{\num{360}} & \significant{\num{162}} & \significant{\num{0.33}} & \significant{\num{0.08}}  & \significant{\num{150}} & \significant{\num{0.31}} & \significant{\num{0.07}} & \significant{\num{152}} & \significant{\num{0.32}} & \significant{\num{0.05}} & \significant{\num{152}} & \significant{\num{0.33}} & \significant{\num{0.09}} & \significant{\num{161}} & \significant{\num{0.33}} & \significant{\num{0.08}}  \\

\bottomrule
\end{tabular}
\end{table*}
\begin{table*}[tbp]
    \centering
    \tiny

    \caption{\mynewcontent{6}{Bug detection summary for each strategy with MOSA}}\label{tab:mosa_bugs}
       \begin{tabular}{llccc|ccc|ccc|ccc|ccc}
\toprule
Project & Bugs & \nrcols{3}{Smart Selection} & \nrcols{3}{Original Combination}  & \nrcols{3}{Branch Coverage} & \nrcols{3}{BC-EC-MC} & \nrcols{3}{SSWS} \\
\cmidrule(l{1pt}r{1pt}){3-5}
\cmidrule(l{1pt}r{1pt}){6-8}
\cmidrule(l{1pt}r{1pt}){9-11}
\cmidrule(l{1pt}r{1pt}){12-14}
\cmidrule(l{1pt}r{1pt}){15-17}
 & & Detected & Detect$\%$ & Fail$\%$ & Detected & Detect$\%$ & Fail$\%$ & Detected & Detect$\%$ & Fail$\%$ & Detected & Detect$\%$ & Fail$\%$ & Detected & Detect$\%$ & Fail$\%$  \\
\midrule


 Chart  & \significant{\num{24}} & \significant{\num{18}} & \significant{\num{0.66}} & \significant{\num{0.05}}  & \significant{\num{16}} & \significant{\num{0.56}} & \significant{\num{0.05}} & \significant{\num{14}} & \significant{\num{0.50}} & \significant{\num{0.02}} & \significant{\num{17}} & \significant{\num{0.63}} & \significant{\num{0.07}} & \significant{\num{19}} & \significant{\num{0.63}} & \significant{\num{0.04}}  \\



\tabprojectlinespace 


 Cli  & \significant{\num{28}} & \significant{\num{17}} & \significant{\num{0.40}} & \significant{\num{0.05}}  & \significant{\num{16}} & \significant{\num{0.39}} & \significant{\num{0.01}} & \significant{\num{16}} & \significant{\num{0.41}} & \significant{\num{0.00}} & \significant{\num{14}} & \significant{\num{0.38}} & \significant{\num{0.00}} & \significant{\num{16}} & \significant{\num{0.43}} & \significant{\num{0.01}}  \\



\tabprojectlinespace 


 Closure  & \significant{\num{38}} & \significant{\num{10}} & \significant{\num{0.14}} & \significant{\num{0.17}}  & \significant{\num{6}} & \significant{\num{0.13}} & \significant{\num{0.16}} & \significant{\num{6}} & \significant{\num{0.07}} & \significant{\num{0.06}} & \significant{\num{9}} & \significant{\num{0.11}} & \significant{\num{0.18}} & \significant{\num{9}} & \significant{\num{0.13}} & \significant{\num{0.18}}  \\



\tabprojectlinespace 


 Compress  & \significant{\num{29}} & \significant{\num{16}} & \significant{\num{0.34}} & \significant{\num{0.07}}  & \significant{\num{14}} & \significant{\num{0.36}} & \significant{\num{0.08}} & \significant{\num{15}} & \significant{\num{0.35}} & \significant{\num{0.03}} & \significant{\num{16}} & \significant{\num{0.43}} & \significant{\num{0.07}} & \significant{\num{14}} & \significant{\num{0.33}} & \significant{\num{0.11}}  \\



\tabprojectlinespace 


 Csv  & \significant{\num{8}} & \significant{\num{5}} & \significant{\num{0.57}} & \significant{\num{0.09}}  & \significant{\num{6}} & \significant{\num{0.59}} & \significant{\num{0.03}} & \significant{\num{6}} & \significant{\num{0.61}} & \significant{\num{0.00}} & \significant{\num{6}} & \significant{\num{0.59}} & \significant{\num{0.04}} & \significant{\num{6}} & \significant{\num{0.65}} & \significant{\num{0.05}}  \\



\tabprojectlinespace 


 Gson  & \significant{\num{14}} & \significant{\num{6}} & \significant{\num{0.34}} & \significant{\num{0.02}}  & \significant{\num{5}} & \significant{\num{0.36}} & \significant{\num{0.04}} & \significant{\num{5}} & \significant{\num{0.33}} & \significant{\num{0.05}} & \significant{\num{5}} & \significant{\num{0.35}} & \significant{\num{0.02}} & \significant{\num{5}} & \significant{\num{0.36}} & \significant{\num{0.02}}  \\



\tabprojectlinespace 


 JacksonCore  & \significant{\num{22}} & \significant{\num{14}} & \significant{\num{0.53}} & \significant{\num{0.05}}  & \significant{\num{15}} & \significant{\num{0.58}} & \significant{\num{0.05}} & \significant{\num{14}} & \significant{\num{0.43}} & \significant{\num{0.08}} & \significant{\num{12}} & \significant{\num{0.40}} & \significant{\num{0.07}} & \significant{\num{14}} & \significant{\num{0.58}} & \significant{\num{0.04}}  \\



\tabprojectlinespace 


 JacksonDatabind  & \significant{\num{75}} & \significant{\num{35}} & \significant{\num{0.27}} & \significant{\num{0.16}}  & \significant{\num{30}} & \significant{\num{0.28}} & \significant{\num{0.11}} & \significant{\num{27}} & \significant{\num{0.25}} & \significant{\num{0.12}} & \significant{\num{27}} & \significant{\num{0.25}} & \significant{\num{0.15}} & \significant{\num{30}} & \significant{\num{0.28}} & \significant{\num{0.14}}  \\



\tabprojectlinespace 


 JacksonXml  & \significant{\num{6}} & \significant{\num{2}} & \significant{\num{0.33}} & \significant{\num{0.02}}  & \significant{\num{2}} & \significant{\num{0.30}} & \significant{\num{0.03}} & \significant{\num{2}} & \significant{\num{0.33}} & \significant{\num{0.07}} & \significant{\num{2}} & \significant{\num{0.32}} & \significant{\num{0.12}} & \significant{\num{2}} & \significant{\num{0.32}} & \significant{\num{0.02}}  \\



\tabprojectlinespace 


 Jsoup  & \significant{\num{58}} & \significant{\num{26}} & \significant{\num{0.32}} & \significant{\num{0.05}}  & \significant{\num{23}} & \significant{\num{0.28}} & \significant{\num{0.05}} & \significant{\num{24}} & \significant{\num{0.30}} & \significant{\num{0.02}} & \significant{\num{23}} & \significant{\num{0.33}} & \significant{\num{0.07}} & \significant{\num{24}} & \significant{\num{0.26}} & \significant{\num{0.04}}  \\



\tabprojectlinespace 


 JxPath  & \significant{\num{12}} & \significant{\num{8}} & \significant{\num{0.41}} & \significant{\num{0.20}}  & \significant{\num{8}} & \significant{\num{0.28}} & \significant{\num{0.17}} & \significant{\num{10}} & \significant{\num{0.57}} & \significant{\num{0.13}} & \significant{\num{10}} & \significant{\num{0.52}} & \significant{\num{0.27}} & \significant{\num{7}} & \significant{\num{0.48}} & \significant{\num{0.33}}  \\



\tabprojectlinespace 


 Lang  & \significant{\num{44}} & \significant{\num{29}} & \significant{\num{0.48}} & \significant{\num{0.05}}  & \significant{\num{22}} & \significant{\num{0.45}} & \significant{\num{0.04}} & \significant{\num{27}} & \significant{\num{0.53}} & \significant{\num{0.02}} & \significant{\num{23}} & \significant{\num{0.45}} & \significant{\num{0.01}} & \significant{\num{28}} & \significant{\num{0.52}} & \significant{\num{0.05}}  \\



\tabprojectlinespace 


 Math  & \significant{\num{2}} & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}}  & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}} & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}} & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}} & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}}  \\



\midrule


 Overall  & \significant{\num{360}} & \significant{\num{187}} & \significant{\num{0.36}} & \significant{\num{0.09}}  & \significant{\num{164}} & \significant{\num{0.35}} & \significant{\num{0.07}} & \significant{\num{167}} & \significant{\num{0.34}} & \significant{\num{0.05}} & \significant{\num{165}} & \significant{\num{0.35}} & \significant{\num{0.09}} & \significant{\num{175}} & \significant{\num{0.37}} & \significant{\num{0.09}}  \\

\bottomrule
\end{tabular}
\end{table*}
\begin{table*}[tbp]
    \centering
    \tiny

    \caption{\mynewcontent{6}{Bug detection summary for each strategy with DynaMOSA}}\label{tab:dynamosa_bugs}
       \begin{tabular}{llccc|ccc|ccc|ccc|ccc}
\toprule
Project & Bugs & \nrcols{3}{Smart Selection} & \nrcols{3}{Original Combination}  & \nrcols{3}{Branch Coverage} & \nrcols{3}{BC-EC-MC} & \nrcols{3}{SSWS} \\
\cmidrule(l{1pt}r{1pt}){3-5}
\cmidrule(l{1pt}r{1pt}){6-8}
\cmidrule(l{1pt}r{1pt}){9-11}
\cmidrule(l{1pt}r{1pt}){12-14}
\cmidrule(l{1pt}r{1pt}){15-17}
 & & Detected & Detect$\%$ & Fail$\%$ & Detected & Detect$\%$ & Fail$\%$ & Detected & Detect$\%$ & Fail$\%$ & Detected & Detect$\%$ & Fail$\%$ & Detected & Detect$\%$ & Fail$\%$  \\
\midrule


 Chart  & \significant{\num{24}} & \significant{\num{18}} & \significant{\num{0.65}} & \significant{\num{0.06}}  & \significant{\num{21}} & \significant{\num{0.68}} & \significant{\num{0.05}} & \significant{\num{16}} & \significant{\num{0.52}} & \significant{\num{0.02}} & \significant{\num{20}} & \significant{\num{0.67}} & \significant{\num{0.08}} & \significant{\num{20}} & \significant{\num{0.64}} & \significant{\num{0.05}}  \\



\tabprojectlinespace 


 Cli  & \significant{\num{28}} & \significant{\num{16}} & \significant{\num{0.44}} & \significant{\num{0.02}}  & \significant{\num{15}} & \significant{\num{0.44}} & \significant{\num{0.01}} & \significant{\num{16}} & \significant{\num{0.41}} & \significant{\num{0.00}} & \significant{\num{15}} & \significant{\num{0.40}} & \significant{\num{0.00}} & \significant{\num{15}} & \significant{\num{0.39}} & \significant{\num{0.00}}  \\



\tabprojectlinespace 


 Closure  & \significant{\num{38}} & \significant{\num{9}} & \significant{\num{0.14}} & \significant{\num{0.21}}  & \significant{\num{10}} & \significant{\num{0.16}} & \significant{\num{0.20}} & \significant{\num{6}} & \significant{\num{0.05}} & \significant{\num{0.06}} & \significant{\num{10}} & \significant{\num{0.11}} & \significant{\num{0.18}} & \significant{\num{9}} & \significant{\num{0.10}} & \significant{\num{0.19}}  \\



\tabprojectlinespace 


 Compress  & \significant{\num{29}} & \significant{\num{14}} & \significant{\num{0.33}} & \significant{\num{0.08}}  & \significant{\num{15}} & \significant{\num{0.36}} & \significant{\num{0.08}} & \significant{\num{13}} & \significant{\num{0.30}} & \significant{\num{0.03}} & \significant{\num{15}} & \significant{\num{0.38}} & \significant{\num{0.04}} & \significant{\num{14}} & \significant{\num{0.36}} & \significant{\num{0.08}}  \\



\tabprojectlinespace 


 Csv  & \significant{\num{8}} & \significant{\num{6}} & \significant{\num{0.64}} & \significant{\num{0.05}}  & \significant{\num{7}} & \significant{\num{0.63}} & \significant{\num{0.05}} & \significant{\num{6}} & \significant{\num{0.61}} & \significant{\num{0.01}} & \significant{\num{5}} & \significant{\num{0.62}} & \significant{\num{0.09}} & \significant{\num{5}} & \significant{\num{0.51}} & \significant{\num{0.05}}  \\



\tabprojectlinespace 


 Gson  & \significant{\num{14}} & \significant{\num{5}} & \significant{\num{0.34}} & \significant{\num{0.01}}  & \significant{\num{5}} & \significant{\num{0.36}} & \significant{\num{0.01}} & \significant{\num{6}} & \significant{\num{0.34}} & \significant{\num{0.06}} & \significant{\num{5}} & \significant{\num{0.36}} & \significant{\num{0.06}} & \significant{\num{5}} & \significant{\num{0.36}} & \significant{\num{0.03}}  \\



\tabprojectlinespace 


 JacksonCore  & \significant{\num{22}} & \significant{\num{13}} & \significant{\num{0.54}} & \significant{\num{0.10}}  & \significant{\num{13}} & \significant{\num{0.52}} & \significant{\num{0.05}} & \significant{\num{13}} & \significant{\num{0.45}} & \significant{\num{0.06}} & \significant{\num{14}} & \significant{\num{0.48}} & \significant{\num{0.07}} & \significant{\num{15}} & \significant{\num{0.53}} & \significant{\num{0.07}}  \\



\tabprojectlinespace 


 JacksonDatabind  & \significant{\num{75}} & \significant{\num{29}} & \significant{\num{0.28}} & \significant{\num{0.14}}  & \significant{\num{33}} & \significant{\num{0.31}} & \significant{\num{0.13}} & \significant{\num{29}} & \significant{\num{0.27}} & \significant{\num{0.12}} & \significant{\num{32}} & \significant{\num{0.29}} & \significant{\num{0.15}} & \significant{\num{30}} & \significant{\num{0.30}} & \significant{\num{0.13}}  \\



\tabprojectlinespace 


 JacksonXml  & \significant{\num{6}} & \significant{\num{2}} & \significant{\num{0.33}} & \significant{\num{0.00}}  & \significant{\num{2}} & \significant{\num{0.32}} & \significant{\num{0.02}} & \significant{\num{2}} & \significant{\num{0.30}} & \significant{\num{0.03}} & \significant{\num{2}} & \significant{\num{0.33}} & \significant{\num{0.03}} & \significant{\num{2}} & \significant{\num{0.33}} & \significant{\num{0.08}}  \\



\tabprojectlinespace 


 Jsoup  & \significant{\num{58}} & \significant{\num{24}} & \significant{\num{0.31}} & \significant{\num{0.04}}  & \significant{\num{23}} & \significant{\num{0.30}} & \significant{\num{0.06}} & \significant{\num{20}} & \significant{\num{0.28}} & \significant{\num{0.02}} & \significant{\num{27}} & \significant{\num{0.33}} & \significant{\num{0.07}} & \significant{\num{27}} & \significant{\num{0.29}} & \significant{\num{0.05}}  \\



\tabprojectlinespace 


 JxPath  & \significant{\num{12}} & \significant{\num{10}} & \significant{\num{0.51}} & \significant{\num{0.23}}  & \significant{\num{8}} & \significant{\num{0.46}} & \significant{\num{0.32}} & \significant{\num{10}} & \significant{\num{0.57}} & \significant{\num{0.17}} & \significant{\num{6}} & \significant{\num{0.38}} & \significant{\num{0.29}} & \significant{\num{9}} & \significant{\num{0.44}} & \significant{\num{0.25}}  \\



\tabprojectlinespace 


 Lang  & \significant{\num{44}} & \significant{\num{25}} & \significant{\num{0.49}} & \significant{\num{0.03}}  & \significant{\num{28}} & \significant{\num{0.55}} & \significant{\num{0.02}} & \significant{\num{22}} & \significant{\num{0.48}} & \significant{\num{0.02}} & \significant{\num{22}} & \significant{\num{0.46}} & \significant{\num{0.01}} & \significant{\num{28}} & \significant{\num{0.51}} & \significant{\num{0.03}}  \\



\tabprojectlinespace 


 Math  & \significant{\num{2}} & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}}  & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}} & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}} & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}} & \significant{\num{1}} & \significant{\num{0.50}} & \significant{\num{0.00}}  \\



\midrule


 Overall  & \significant{\num{360}} & \significant{\num{172}} & \significant{\num{0.37}} & \significant{\num{0.09}}  & \significant{\num{181}} & \significant{\num{0.39}} & \significant{\num{0.09}} & \significant{\num{160}} & \significant{\num{0.34}} & \significant{\num{0.05}} & \significant{\num{174}} & \significant{\num{0.37}} & \significant{\num{0.09}} & \significant{\num{180}} & \significant{\num{0.37}} & \significant{\num{0.09}}  \\

\bottomrule
\end{tabular}
\end{table*}


==> tab/classes.tex <==

\begin{table*}[tbp]
    \centering
    \footnotesize

    \caption{Overview of Java projects and classes in our evaluation}
    \label{tab:classes}

   \begin{tabular}{lllllllll}
\toprule
Project & Package & Classes & \nrcols{3}{Branch} & \nrcols{3}{\mynewcontent{6}{Statement}} \\
\cmidrule(l{1pt}r{1pt}){4-6}
\cmidrule(l{1pt}r{1pt}){7-9}
& & & $25\%$ & mean & $75\%$ & $25\%$ & mean & $75\%$  \\
\midrule

 a4j & \priostrategy{-} & \significant{\num{1}} & \significant{\num{125}} & \significant{\num{125}} & \significant{\num{125}}  & \significant{\num{2038}} & \significant{\num{2038}} & \significant{\num{2038}}  \\

\tabprojectlinespace 
 
 apbsmem & \priostrategy{-} & \significant{\num{1}} & \significant{\num{390}} & \significant{\num{390}} & \significant{\num{390}}  & \significant{\num{4323}} & \significant{\num{4323}} & \significant{\num{4323}}  \\

\tabprojectlinespace 
 
 at-robots2-j & \priostrategy{-} & \significant{\num{1}} & \significant{\num{125}} & \significant{\num{125}} & \significant{\num{125}}  & \significant{\num{832}} & \significant{\num{832}} & \significant{\num{832}}  \\

\tabprojectlinespace 
 
 battlecry & \priostrategy{-} & \significant{\num{2}} & \significant{\num{128}} & \significant{\num{179}} & \significant{\num{230}}  & \significant{\num{1767}} & \significant{\num{1947}} & \significant{\num{2126}}  \\

\tabprojectlinespace 
 
 biff & \priostrategy{-} & \significant{\num{1}} & \significant{\num{817}} & \significant{\num{817}} & \significant{\num{817}}  & \significant{\num{7012}} & \significant{\num{7012}} & \significant{\num{7012}}  \\

\tabprojectlinespace 
 
 caloriecount & \priostrategy{-} & \significant{\num{1}} & \significant{\num{232}} & \significant{\num{232}} & \significant{\num{232}}  & \significant{\num{1425}} & \significant{\num{1425}} & \significant{\num{1425}}  \\

\tabprojectlinespace 
 
 celwars2009 & \priostrategy{-} & \significant{\num{1}} & \significant{\num{360}} & \significant{\num{360}} & \significant{\num{360}}  & \significant{\num{2139}} & \significant{\num{2139}} & \significant{\num{2139}}  \\

\tabprojectlinespace 
 
 checkstyle & \priostrategy{-} & \significant{\num{1}} & \significant{\num{50}} & \significant{\num{50}} & \significant{\num{50}}  & \significant{\num{412}} & \significant{\num{412}} & \significant{\num{412}}  \\

\tabprojectlinespace 
 
 classviewer & \priostrategy{-} & \significant{\num{3}} & \significant{\num{114}} & \significant{\num{154}} & \significant{\num{202}}  & \significant{\num{671}} & \significant{\num{1219}} & \significant{\num{1665}}  \\

\tabprojectlinespace 
 
 commons-cli & \priostrategy{-} & \significant{\num{2}} & \significant{\num{139}} & \significant{\num{146}} & \significant{\num{152}}  & \significant{\num{696}} & \significant{\num{788}} & \significant{\num{880}}  \\

\tabprojectlinespace 
 
 commons-codec & \priostrategy{-} & \significant{\num{1}} & \significant{\num{504}} & \significant{\num{504}} & \significant{\num{504}}  & \significant{\num{2385}} & \significant{\num{2385}} & \significant{\num{2385}}  \\

\tabprojectlinespace 
 
 commons-collections & \priostrategy{-} & \significant{\num{2}} & \significant{\num{122}} & \significant{\num{155}} & \significant{\num{188}}  & \significant{\num{351}} & \significant{\num{426}} & \significant{\num{501}}  \\

\tabprojectlinespace 
 
 commons-lang & \priostrategy{-} & \significant{\num{12}} & \significant{\num{137}} & \significant{\num{353}} & \significant{\num{370}}  & \significant{\num{868}} & \significant{\num{1759}} & \significant{\num{2037}}  \\

\tabprojectlinespace 
 
 commons-math & \priostrategy{-} & \significant{\num{17}} & \significant{\num{75}} & \significant{\num{120}} & \significant{\num{149}}  & \significant{\num{630}} & \significant{\num{1105}} & \significant{\num{1350}}  \\

\tabprojectlinespace 
 
 corina & \priostrategy{-} & \significant{\num{1}} & \significant{\num{55}} & \significant{\num{55}} & \significant{\num{55}}  & \significant{\num{282}} & \significant{\num{282}} & \significant{\num{282}}  \\

\tabprojectlinespace 
 
 dcparseargs & \priostrategy{-} & \significant{\num{1}} & \significant{\num{80}} & \significant{\num{80}} & \significant{\num{80}}  & \significant{\num{571}} & \significant{\num{571}} & \significant{\num{571}}  \\

\tabprojectlinespace 
 
 dsachat & \priostrategy{-} & \significant{\num{2}} & \significant{\num{76}} & \significant{\num{83}} & \significant{\num{90}}  & \significant{\num{868}} & \significant{\num{880}} & \significant{\num{892}}  \\

\tabprojectlinespace 
 
 dvd-homevideo & \priostrategy{-} & \significant{\num{2}} & \significant{\num{60}} & \significant{\num{68}} & \significant{\num{76}}  & \significant{\num{1269}} & \significant{\num{1308}} & \significant{\num{1347}}  \\

\tabprojectlinespace 
 
 feudalismgame & \priostrategy{-} & \significant{\num{1}} & \significant{\num{788}} & \significant{\num{788}} & \significant{\num{788}}  & \significant{\num{4873}} & \significant{\num{4873}} & \significant{\num{4873}}  \\

\tabprojectlinespace 
 
 fim1 & \priostrategy{-} & \significant{\num{1}} & \significant{\num{73}} & \significant{\num{73}} & \significant{\num{73}}  & \significant{\num{1140}} & \significant{\num{1140}} & \significant{\num{1140}}  \\

\tabprojectlinespace 
 
 firebird & \priostrategy{-} & \significant{\num{2}} & \significant{\num{123}} & \significant{\num{147}} & \significant{\num{171}}  & \significant{\num{666}} & \significant{\num{751}} & \significant{\num{836}}  \\

\tabprojectlinespace 
 
 fixsuite & \priostrategy{-} & \significant{\num{1}} & \significant{\num{74}} & \significant{\num{74}} & \significant{\num{74}}  & \significant{\num{631}} & \significant{\num{631}} & \significant{\num{631}}  \\

\tabprojectlinespace 
 
 fps370 & \priostrategy{-} & \significant{\num{1}} & \significant{\num{70}} & \significant{\num{70}} & \significant{\num{70}}  & \significant{\num{668}} & \significant{\num{668}} & \significant{\num{668}}  \\

\tabprojectlinespace 
 
 freemind & \priostrategy{-} & \significant{\num{1}} & \significant{\num{208}} & \significant{\num{208}} & \significant{\num{208}}  & \significant{\num{1621}} & \significant{\num{1621}} & \significant{\num{1621}}  \\

\tabprojectlinespace 
 
 gfarcegestionfa & \priostrategy{-} & \significant{\num{2}} & \significant{\num{87}} & \significant{\num{99}} & \significant{\num{111}}  & \significant{\num{664}} & \significant{\num{826}} & \significant{\num{988}}  \\

\tabprojectlinespace 
 
 glengineer & \priostrategy{-} & \significant{\num{1}} & \significant{\num{115}} & \significant{\num{115}} & \significant{\num{115}}  & \significant{\num{658}} & \significant{\num{658}} & \significant{\num{658}}  \\

\tabprojectlinespace 
 
 guava & \priostrategy{-} & \significant{\num{8}} & \significant{\num{84}} & \significant{\num{143}} & \significant{\num{160}}  & \significant{\num{213}} & \significant{\num{490}} & \significant{\num{742}}  \\

\tabprojectlinespace 
  
 httpanalyzer & \priostrategy{-} & \significant{\num{1}} & \significant{\num{56}} & \significant{\num{56}} & \significant{\num{56}}  & \significant{\num{656}} & \significant{\num{656}} & \significant{\num{656}}  \\

\tabprojectlinespace 
 
 ifx-framework & \priostrategy{-} & \significant{\num{1}} & \significant{\num{72}} & \significant{\num{72}} & \significant{\num{72}}  & \significant{\num{462}} & \significant{\num{462}} & \significant{\num{462}}  \\

\tabprojectlinespace 
 
 inspirento & \priostrategy{-} & \significant{\num{1}} & \significant{\num{95}} & \significant{\num{95}} & \significant{\num{95}}  & \significant{\num{649}} & \significant{\num{649}} & \significant{\num{649}}  \\

\tabprojectlinespace 
 
 io-project & \priostrategy{-} & \significant{\num{1}} & \significant{\num{66}} & \significant{\num{66}} & \significant{\num{66}}  & \significant{\num{282}} & \significant{\num{282}} & \significant{\num{282}}  \\

\tabprojectlinespace 
 
 ipcalculator & \priostrategy{-} & \significant{\num{2}} & \significant{\num{67}} & \significant{\num{79}} & \significant{\num{91}}  & \significant{\num{1164}} & \significant{\num{1252}} & \significant{\num{1340}}  \\

\tabprojectlinespace 
 
 javaml & \priostrategy{-} & \significant{\num{3}} & \significant{\num{51}} & \significant{\num{52}} & \significant{\num{54}}  & \significant{\num{390}} & \significant{\num{409}} & \significant{\num{424}}  \\

\tabprojectlinespace 
 
 javathena & \priostrategy{-} & \significant{\num{1}} & \significant{\num{255}} & \significant{\num{255}} & \significant{\num{255}}  & \significant{\num{2278}} & \significant{\num{2278}} & \significant{\num{2278}}  \\

\tabprojectlinespace 
 
 javaviewcontrol & \priostrategy{-} & \significant{\num{2}} & \significant{\num{760}} & \significant{\num{1298}} & \significant{\num{1835}}  & \significant{\num{3078}} & \significant{\num{4394}} & \significant{\num{5710}}  \\

\tabprojectlinespace 
 
 jclo & \priostrategy{-} & \significant{\num{1}} & \significant{\num{133}} & \significant{\num{133}} & \significant{\num{133}}  & \significant{\num{987}} & \significant{\num{987}} & \significant{\num{987}}  \\

\tabprojectlinespace 
 
 jcvi-javacommon & \priostrategy{-} & \significant{\num{1}} & \significant{\num{61}} & \significant{\num{61}} & \significant{\num{61}}  & \significant{\num{240}} & \significant{\num{240}} & \significant{\num{240}}  \\

\tabprojectlinespace 
 
 jdom & \priostrategy{-} & \significant{\num{5}} & \significant{\num{63}} & \significant{\num{110}} & \significant{\num{91}}  & \significant{\num{510}} & \significant{\num{591}} & \significant{\num{583}}  \\

\tabprojectlinespace 
 
 jfreechart & \priostrategy{-} & \significant{\num{8}} & \significant{\num{102}} & \significant{\num{263}} & \significant{\num{242}}  & \significant{\num{754}} & \significant{\num{1881}} & \significant{\num{1843}}  \\

\tabprojectlinespace 
 
 jiggler & \priostrategy{-} & \significant{\num{3}} & \significant{\num{65}} & \significant{\num{82}} & \significant{\num{96}}  & \significant{\num{465}} & \significant{\num{711}} & \significant{\num{836}}  \\

\tabprojectlinespace 
 
 jipa & \priostrategy{-} & \significant{\num{1}} & \significant{\num{134}} & \significant{\num{134}} & \significant{\num{134}}  & \significant{\num{783}} & \significant{\num{783}} & \significant{\num{783}}  \\

\tabprojectlinespace 
 
 jiprof & \priostrategy{-} & \significant{\num{4}} & \significant{\num{84}} & \significant{\num{451}} & \significant{\num{818}}  & \significant{\num{628}} & \significant{\num{2612}} & \significant{\num{4344}}  \\

\tabprojectlinespace 
 
 jmca & \priostrategy{-} & \significant{\num{3}} & \significant{\num{207}} & \significant{\num{707}} & \significant{\num{961}}  & \significant{\num{1122}} & \significant{\num{2307}} & \significant{\num{2978}}  \\

\tabprojectlinespace 
  
 jopenchart & \priostrategy{-} & \significant{\num{1}} & \significant{\num{92}} & \significant{\num{92}} & \significant{\num{92}}  & \significant{\num{1139}} & \significant{\num{1139}} & \significant{\num{1139}}  \\

\tabprojectlinespace 

hadoop & \priostrategy{org} & \significant{\num{45}} & \significant{\num{70}} & \significant{\num{151}} & \significant{\num{156}}  & \significant{\num{121}} & \significant{\num{271}} & \significant{\num{313}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache} & \significant{\num{65}} & \significant{\num{70}} & \significant{\num{343}} & \significant{\num{158}}  & \significant{\num{105}} & \significant{\num{565}} & \significant{\num{295}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop} & \significant{\num{40}} & \significant{\num{62}} & \significant{\num{220}} & \significant{\num{194}}  & \significant{\num{133}} & \significant{\num{403}} & \significant{\num{331}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.crypto} & \significant{\num{1}} & \significant{\num{82}} & \significant{\num{82}} & \significant{\num{82}}  & \significant{\num{337}} & \significant{\num{337}} & \significant{\num{337}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.mapreduce} & \significant{\num{3}} & \significant{\num{78}} & \significant{\num{90}} & \significant{\num{101}}  & \significant{\num{184}} & \significant{\num{204}} & \significant{\num{218}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.mapreduce.v2.api} & \significant{\num{3}} & \significant{\num{80}} & \significant{\num{91}} & \significant{\num{110}}  & \significant{\num{136}} & \significant{\num{160}} & \significant{\num{196}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.security} & \significant{\num{1}} & \significant{\num{74}} & \significant{\num{74}} & \significant{\num{74}}  & \significant{\num{159}} & \significant{\num{159}} & \significant{\num{159}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.thirdparty.com} & \significant{\num{18}} & \significant{\num{71}} & \significant{\num{108}} & \significant{\num{122}}  & \significant{\num{108}} & \significant{\num{154}} & \significant{\num{174}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.thirdparty.com.google} & \significant{\num{4}} & \significant{\num{74}} & \significant{\num{114}} & \significant{\num{127}}  & \significant{\num{141}} & \significant{\num{196}} & \significant{\num{239}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.thirdparty.org} & \significant{\num{1}} & \significant{\num{119}} & \significant{\num{119}} & \significant{\num{119}}  & \significant{\num{163}} & \significant{\num{163}} & \significant{\num{163}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.yarn} & \significant{\num{22}} & \significant{\num{59}} & \significant{\num{103}} & \significant{\num{117}}  & \significant{\num{99}} & \significant{\num{186}} & \significant{\num{208}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.yarn.api} & \significant{\num{14}} & \significant{\num{56}} & \significant{\num{107}} & \significant{\num{134}}  & \significant{\num{106}} & \significant{\num{183}} & \significant{\num{212}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.yarn.server} & \significant{\num{11}} & \significant{\num{55}} & \significant{\num{105}} & \significant{\num{101}}  & \significant{\num{98}} & \significant{\num{193}} & \significant{\num{191}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.yarn.server.api} & \significant{\num{4}} & \significant{\num{95}} & \significant{\num{117}} & \significant{\num{138}}  & \significant{\num{176}} & \significant{\num{208}} & \significant{\num{242}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.yarn.server.applicationhistoryservice} & \significant{\num{1}} & \significant{\num{55}} & \significant{\num{55}} & \significant{\num{55}}  & \significant{\num{95}} & \significant{\num{95}} & \significant{\num{95}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.yarn.server.federation.store} & \significant{\num{1}} & \significant{\num{69}} & \significant{\num{69}} & \significant{\num{69}}  & \significant{\num{109}} & \significant{\num{109}} & \significant{\num{109}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.yarn.server.nodemanager} & \significant{\num{2}} & \significant{\num{84}} & \significant{\num{91}} & \significant{\num{98}}  & \significant{\num{170}} & \significant{\num{187}} & \significant{\num{204}}  \\

\tabprojectlinespace 
 
 hadoop & \priostrategy{org.apache.hadoop.yarn.server.nodemanager.containermanager} & \significant{\num{4}} & \significant{\num{59}} & \significant{\num{60}} & \significant{\num{63}}  & \significant{\num{99}} & \significant{\num{112}} & \significant{\num{131}}  \\

\tabprojectlinespace 


\end{tabular}

\end{table*}


\begin{table*}[tbp]
\ContinuedFloat
    \centering
    \footnotesize
    \caption{Continued}
    \label{tab:classes_2}

   \begin{tabular}{lp{8cm}lllllll}
\toprule
Project & Package & Classes & \nrcols{3}{Branch} & \nrcols{3}{Statement} \\
\cmidrule(l{1pt}r{1pt}){4-6}
\cmidrule(l{1pt}r{1pt}){7-9}
& & & $25\%$ & mean & $75\%$ & $25\%$ & mean & $75\%$  \\
\midrule
 
 hadoop & \priostrategy{org.apache.hadoop.yarn.server.resourcemanager} & \significant{\num{2}} & \significant{\num{106}} & \significant{\num{127}} & \significant{\num{147}}  & \significant{\num{246}} & \significant{\num{281}} & \significant{\num{315}}  \\

\tabprojectlinespace
 
 jsecurity & \priostrategy{-} & \significant{\num{1}} & \significant{\num{170}} & \significant{\num{170}} & \significant{\num{170}}  & \significant{\num{725}} & \significant{\num{725}} & \significant{\num{725}}  \\

\tabprojectlinespace 
 
 lagoon & \priostrategy{-} & \significant{\num{2}} & \significant{\num{63}} & \significant{\num{64}} & \significant{\num{64}}  & \significant{\num{758}} & \significant{\num{841}} & \significant{\num{924}}  \\

\tabprojectlinespace 
 
 lhamacaw & \priostrategy{-} & \significant{\num{1}} & \significant{\num{70}} & \significant{\num{70}} & \significant{\num{70}}  & \significant{\num{714}} & \significant{\num{714}} & \significant{\num{714}}  \\

\tabprojectlinespace 
 
 liferay & \priostrategy{-} & \significant{\num{1}} & \significant{\num{78}} & \significant{\num{78}} & \significant{\num{78}}  & \significant{\num{462}} & \significant{\num{462}} & \significant{\num{462}}  \\

\tabprojectlinespace 
 
 lilith & \priostrategy{-} & \significant{\num{1}} & \significant{\num{134}} & \significant{\num{134}} & \significant{\num{134}}  & \significant{\num{496}} & \significant{\num{496}} & \significant{\num{496}}  \\

\tabprojectlinespace 
 
 newzgrabber & \priostrategy{-} & \significant{\num{2}} & \significant{\num{125}} & \significant{\num{173}} & \significant{\num{220}}  & \significant{\num{1110}} & \significant{\num{1257}} & \significant{\num{1404}}  \\

\tabprojectlinespace 
 
 noen & \priostrategy{-} & \significant{\num{2}} & \significant{\num{68}} & \significant{\num{69}} & \significant{\num{70}}  & \significant{\num{386}} & \significant{\num{456}} & \significant{\num{526}}  \\

\tabprojectlinespace 
 
 objectexplorer & \priostrategy{-} & \significant{\num{1}} & \significant{\num{175}} & \significant{\num{175}} & \significant{\num{175}}  & \significant{\num{987}} & \significant{\num{987}} & \significant{\num{987}}  \\

\tabprojectlinespace 
 
 openhre & \priostrategy{-} & \significant{\num{1}} & \significant{\num{50}} & \significant{\num{50}} & \significant{\num{50}}  & \significant{\num{220}} & \significant{\num{220}} & \significant{\num{220}}  \\

\tabprojectlinespace 
 
 quickserver & \priostrategy{-} & \significant{\num{2}} & \significant{\num{70}} & \significant{\num{71}} & \significant{\num{72}}  & \significant{\num{553}} & \significant{\num{618}} & \significant{\num{683}}  \\

\tabprojectlinespace 
 
 resources4j & \priostrategy{-} & \significant{\num{1}} & \significant{\num{176}} & \significant{\num{176}} & \significant{\num{176}}  & \significant{\num{1539}} & \significant{\num{1539}} & \significant{\num{1539}}  \\

\tabprojectlinespace 
 
 saxpath & \priostrategy{-} & \significant{\num{2}} & \significant{\num{162}} & \significant{\num{269}} & \significant{\num{376}}  & \significant{\num{344}} & \significant{\num{574}} & \significant{\num{804}}  \\

\tabprojectlinespace 
 
 schemaspy & \priostrategy{-} & \significant{\num{1}} & \significant{\num{380}} & \significant{\num{380}} & \significant{\num{380}}  & \significant{\num{2241}} & \significant{\num{2241}} & \significant{\num{2241}}  \\

\tabprojectlinespace 
 
 shop & \priostrategy{-} & \significant{\num{3}} & \significant{\num{100}} & \significant{\num{131}} & \significant{\num{153}}  & \significant{\num{833}} & \significant{\num{998}} & \significant{\num{1145}}  \\

\tabprojectlinespace 
 
 sugar & \priostrategy{-} & \significant{\num{1}} & \significant{\num{51}} & \significant{\num{51}} & \significant{\num{51}}  & \significant{\num{484}} & \significant{\num{484}} & \significant{\num{484}}  \\

\tabprojectlinespace 
 
 summa & \priostrategy{-} & \significant{\num{1}} & \significant{\num{372}} & \significant{\num{372}} & \significant{\num{372}}  & \significant{\num{1906}} & \significant{\num{1906}} & \significant{\num{1906}}  \\

\tabprojectlinespace 
 
 sweethome3d & \priostrategy{-} & \significant{\num{2}} & \significant{\num{271}} & \significant{\num{387}} & \significant{\num{503}}  & \significant{\num{1544}} & \significant{\num{2152}} & \significant{\num{2760}}  \\

\tabprojectlinespace 
 
 trove & \priostrategy{-} & \significant{\num{9}} & \significant{\num{77}} & \significant{\num{137}} & \significant{\num{255}}  & \significant{\num{378}} & \significant{\num{652}} & \significant{\num{852}}  \\

\tabprojectlinespace 
 
 twfbplayer & \priostrategy{-} & \significant{\num{2}} & \significant{\num{94}} & \significant{\num{115}} & \significant{\num{135}}  & \significant{\num{631}} & \significant{\num{839}} & \significant{\num{1047}}  \\

\tabprojectlinespace 
 
 twitter4j & \priostrategy{-} & \significant{\num{6}} & \significant{\num{64}} & \significant{\num{117}} & \significant{\num{115}}  & \significant{\num{399}} & \significant{\num{1493}} & \significant{\num{823}}  \\

\tabprojectlinespace 
 
 vuze & \priostrategy{-} & \significant{\num{1}} & \significant{\num{134}} & \significant{\num{134}} & \significant{\num{134}}  & \significant{\num{675}} & \significant{\num{675}} & \significant{\num{675}}  \\

\tabprojectlinespace 
 
 weka & \priostrategy{-} & \significant{\num{3}} & \significant{\num{257}} & \significant{\num{441}} & \significant{\num{538}}  & \significant{\num{1505}} & \significant{\num{3606}} & \significant{\num{4777}}  \\

\tabprojectlinespace 
 
 wheelwebtool & \priostrategy{-} & \significant{\num{3}} & \significant{\num{116}} & \significant{\num{349}} & \significant{\num{495}}  & \significant{\num{1031}} & \significant{\num{2002}} & \significant{\num{2817}}  \\
 

\midrule

Overall
& \priostrategy{-}  & \significant{\num{400}} & \significant{\num{67}} & \significant{\num{201}} & \significant{\num{171}}  & \significant{\num{144}} & \significant{\num{725}} & \significant{\num{749}} \\

\bottomrule
\end{tabular}

\end{table*}

